Emergent organization of receptive fields in networks of excitatory and inhibitory neurons

Local patterns of excitation and inhibition that can generate neural waves are studied as a computational mechanism underlying the organization of neuronal tunings. Sparse coding algorithms based on networks of excitatory and inhibitory neurons are proposed that exhibit topographic maps as the receptive fields are adapted to input stimuli. Motivated by a leaky integrate-and-fire model of neural waves, we propose an activation model that is more typical of artificial neural networks. Computational experiments with the activation model using both natural images and natural language text are presented. In the case of images, familiar "pinwheel" patterns of oriented edge detectors emerge; in the case of text, the resulting topographic maps exhibit a 2-dimensional representation of granular word semantics. Experiments with a synthetic model of somatosensory input are used to investigate how the network dynamics may affect plasticity of neuronal maps under changes to the inputs.

==> additional.tex <==

% !TEX root = surfing.tex

\section{Additional Simulations}
\label{sec:addsims}

Here we give additional plots for experiments comparing surfing over a sequence of networks during training to gradient descent over the final trained network. As described in the main text,
we consider the problem of minimizing the objective $f(x) = \frac{1}{2}\|G(x) - G(x_*)\|^2$, that is, recovering the image generated from a trained network $G(x) = G_{\theta_T}(x)$ with input $x_*$. We run surfing by taking a sequence of parameters $\theta_0, \theta_1,...,\theta_T$, where $\theta_0$ are the initial random parameters and the intermediate $\theta_t$'s are taken every 40 training steps. In order to improve convergence speed we use Adam \citep{kingma2014adam} to carry out gradient descent in each step in surfing. We also use Adam when optimizing over the just the final network. We apply surfing and regular Adam for 300 trials, where in each trial a randomly generated $x_*$ and initial point $x_{init}$ is chosen. Figure \ref{fig:more} shows
the distribution of the distance between the computed solution $\hat x_T$ and the truth $x_*$ for VAE, WGAN and WGAN-GP,
using surfing (red) and regular gradient descent with Adam (blue), over three different input dimensions $k$.

\begin{figure}[h]
\begin{center}
\begin{tabular}{ccc}
  \\[20pt]
\includegraphics[width=.3\textwidth]{newfigs/VAEdim-5} &
\includegraphics[width=.3\textwidth]{newfigs/VAEdim-10} &
\includegraphics[width=.3\textwidth]{newfigs/VAEdim-20} \\
\includegraphics[width=.3\textwidth]{newfigs/WGANdim-5} &
\includegraphics[width=.3\textwidth]{newfigs/WGANdim-10} &
\includegraphics[width=.3\textwidth]{newfigs/WGANdim-20}\\
\includegraphics[width=.3\textwidth]{newfigs/WGAN-GPdim-5} &
\includegraphics[width=.3\textwidth]{newfigs/WGAN-GPdim-10} &
\includegraphics[width=.3\textwidth]{newfigs/WGAN-GPdim-20}
\end{tabular}
\end{center}
\caption{Distribution of the distance between solution $\hat x_T$ and the truth $x_*$ for VAE, WGAN and WGAN-GP,
using surfing (red) and regular gradient descent with Adam (blue) over three different input dimensions $k$.}
\label{fig:more}
\end{figure}


==> experiments.tex <==
% !TEX root = surfing.tex

\def\R{{\mathbb R}}

\section{Experiments}
\label{sec:experiments}


\afterpage{
\begin{table}[t!]
\begin{center}
\vskip-20pt
\begin{tabular}{|l||l|ccc|ccc|}
\hline
 Input dimension    & & 5       & 10      & 20
& 5       & 10    & 20  \\
\hline \hline
& Model & \multicolumn{3}{c|}{VAE}   & \multicolumn{3}{c|}{DCGAN} \\
\hline
    \multirow{2}{*}{\% successful}    & Regular Adam & 98.7 & 100 & 100 & 48.3    & 68.7 & 80.0\\
    & Surfing    & 100 & 100 & 100 & 78.3    & 98.7    & 96.3 \\
\hline
    \multirow{2}{*}{\# iterations}    & Regular Adam  & 737 & 1330 & 8215 & 618    & 4560 & 18937 \\
    & Surfing     & 775 & 1404 & 10744 & 741    & 6514    & 33294 \\
\hline \hline
& Model & 
\multicolumn{3}{c|}{WGAN} & \multicolumn{3}{c|}{WGAN-GP} \\
\hline
    \multirow{2}{*}{\% successful}    & Regular Adam  & 56.0    & 84.3  & 90.3  & 47.0    & 64.7    & 64.7   \\
    & Surfing      & 81.7    & 97.3  & 99.3   & 83.7    & 95.7    & 97.3 \\
\hline
    \multirow{2}{*}{\# iterations}    & Regular Adam  & 464    & 1227  & 3702  & 463    & 1915    & 15445   \\
    & Surfing   & 547    & 1450  & 4986   & 564    & 2394    & 25991 \\
\hline
\end{tabular}
\end{center}
\vskip5pt
\caption{Surfing compared against direct gradient descent over the final trained
    network, for various generative models with input dimensions $k=5,10,20$. Shown are percentages of ``successful'' solutions $\hat x_T$
    satisfying $\|\hat x_T - x_*\| < 0.01$, and 75th-percentiles of the total
    number of gradient descent steps used (across all networks $G_0,\ldots,G_T$
    for surfing) until $\|\hat x_T - x_*\| < 0.01$ was reached.}
\label{table:prop}
\vskip-10pt
\end{table}

\begin{figure}[h!]
  \begin{center}
  \begin{tabular}{ccc}
  \includegraphics[width=.3\textwidth]{newfigs/DCGANdim-5} &
  \includegraphics[width=.3\textwidth]{newfigs/DCGANdim-10} &
  \includegraphics[width=.3\textwidth]{newfigs/DCGANdim-20} \\[-10pt]
  \end{tabular}
  \end{center}
  \caption{Distribution of distance between solution $\hat x_T$ and the truth $x_*$ for DCGAN trained models, comparing surfing (red) to regular gradient descent (blue) over the final network. Both procedures use Adam in their gradient descent computations. The results indicate that direct descent often succeeds, but can also converge to a point that is far from the optimum. By moving along the optimum of the evolving surface, surfing is able to move closer to the optimum in these cases.}
  \vskip18pt
    \label{fig:dist-WGAN}
  \end{figure}
}

We present experiments to illustrate the performance of surfing over a sequence of networks during training compared with gradient descent over the final trained network. We mainly use the Fashion-MNIST dataset %\footnote{https://github.com/zalandoresearch/fashion-mnist}
to carry out the simulations, which is similar
to MNIST in many characteristics, but is more difficult to train. We build multiple generative models, trained using VAE \citep{kingma2013auto}, DCGAN \citep{radford2015unsupervised}, WGAN \citep{arjovsky2017wasserstein} and WGAN-GP \citep{gulrajani2017improved}. The structure of the generator/decoder networks that we use are the same as those reported by  \cite{chen2016infogan}; they include two fully connected layers and two transposed convolution layers with batch normalization after each layer \citep{ioffe2015batch}. We use the simple surfing algorithm in these experiments, rather than the projected-gradient algorithm proposed for theoretical analysis. Note also that the network architectures do not precisely match the expansive ReLU networks used in our analysis. Instead, we experiment with architectures and training procedures that are meant to better reflect the current state of the art.

We first consider the problem of minimizing the objective $f(x) =
\frac{1}{2}\|G(x) - G(x_*)\|^2$ and recovering the image generated from a
trained network $G(x) = G_{\theta_T}(x)$ with input $x_*$. We run surfing by
taking a sequence of parameters $\theta_0, \theta_1,...,\theta_T$ for $T=100$, where
$\theta_0$ are the initial random parameters and the intermediate $\theta_t$'s
are taken every 40 training steps, and we use
Adam \citep{kingma2014adam} to carry out gradient descent in $x$ over each
network $G_{\theta_t}$. We compare this to ``regular Adam'', which uses Adam to
optimize over $x$ in only  the final trained network $G_{\theta_T}$ for $T=100$.

To ensure that the runtime of surfing is comparable to that of a single
initialization of regular Adam, we do not run Adam until
convergence for each intermediate network in surfing. Instead, we use a fixed
schedule of iterations for the networks $G_{\theta_0},\ldots,G_{\theta_{T-1}}$,
and run Adam to convergence in only the final network $G_{\theta_T}$.
The total number of iterations for networks
$G_{\theta_0},\ldots,G_{\theta_{T-1}}$ is set as the
75th-percentile of the iteration count required for convergence of regular Adam.
These are split across the networks proportional to a deterministic
schedule that allots more steps to the earlier networks where the landscape of
$G(x)$ changes more rapidly, and fewer steps to later networks where this landscape stabilizes.

\newpage
For each network training condition, we apply surfing and regular Adam for 300
trials, where in each trial a randomly generated $x_*$ and initial point
$x_{init}$ are chosen uniformly from the hypercube $[-1,1]^k$. Table
\ref{table:prop} shows the percentage of trials where the solutions $\hat x_T$
satisfy our criterion for successful recovery $\|\hat x_T - x_*\| < 0.01$, for different
models and over three different input dimensions $k$. The table also shows the
75th-percentile for the total number of gradient descent iterations taken
(across all networks for surfing), verifying that the runtime of surfing was
typically 1--2x that of regular Adam. We also provide the distributions of
$\|\hat x_T - x_*\|$ under each setting: Figure \ref{fig:dist-WGAN} shows the
results for DCGAN, and results for the other models are collected in the supplementary material.

We next consider the compressed sensing problem with objective $f(x) = \frac{1}{2}\|AG(x) - AG(x_*)\|^2$ where $A\in\R^{m\times n}$ is the Gaussian measurement matrix. We carry out 200 trials for each choice of number of measurements $m$. The parameters $\theta_t$ for surfing are taken every 100 training steps. As before, we record the proportion of the solutions that are close to the truth $x_*$ according to $\|\hat x_T - x_*\| < 0.01$. Figure \ref{fig:prop} shows the results for DCGAN and WGAN trained networks with input dimension $k=20$.


Lastly, we consider the objective $f(x) = \frac{1}{2}\|AG(x) - Ay\|^2$, where $y$ is a real image from the hold-out test data.
This can be thought of as a rate-distortion setting, where the error varies as a function of the number of measurements used.
We carry out the same experiments as before and compute the average per-pixel reconstruction error $\sqrt{\frac{1}{n}\|G(\hat x_T) - y\|^2}$ as in \cite{bora2017compressed}. Figure \ref{fig:reconstr} shows the distributions of the reconstruction error as the number of measurements $m$ varies.

\begin{figure}
  \begin{center}
  \begin{tabular}{cc}
  \includegraphics[width=.40\textwidth]{newfigs/DCGAN-thres} &
  \includegraphics[width=.40\textwidth]{newfigs/WGAN-thres} \\[-10pt]
  \end{tabular}
  \end{center}
  \caption{Compressed sensing setting for exact recovery. As a function of the number
  of random measurements $m$, the lines show the proportion of times surfing (red) and
  regular gradient descent with Adam (blue) are able to recover the true signal $y = G(x)$, using DCGAN and WGAN.}
  \label{fig:prop}
\vskip10pt
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=.40\textwidth]{newfigs/DCGAN-comp} &
\includegraphics[width=.40\textwidth]{newfigs/WGAN-comp} \\[-10pt]
\end{tabular}
\end{center}
\caption{Compressed sensing setting for approximation, or rate-distortion.
As a function of the number
of random measurements $m$, the box plots summarize the distribution of the per-pixel reconstruction errors for DCGAN and WGAN trained models, using surfing (red) and regular gradient descent with Adam (blue). }
\label{fig:reconstr}
\end{figure}

